Inverse Elastica: A Theoretical Framework for Inverse Design of Morphing Slender Structures

Inverse design of morphing slender structures with programmable curvature has significant applications in various engineering fields. Most existing studies formulate it as an optimization problem, which requires repeatedly solving the forward equations to identify optimal designs. Such methods, however, are computationally intensive and often susceptible to local minima issues. In contrast, solving the inverse problem theoretically, which can bypass the need for optimizations, is highly efficient yet remains challenging, particularly for cases involving arbitrary boundary conditions (BCs). Here, we develop a systematic theoretical framework, termed inverse elastica, for the direct determination of the undeformed configuration from a target deformed shape along with prescribed BCs. Building upon the classical elastica, inverse elastica is derived by supplementing the geometric equations of undeformed configurations. The framework shows three key features: reduced nonlinearity, solution multiplicity, and inverse loading. These principles are demonstrated through two representative models: an analytical solution for a two-dimensional arc and a numerical continuation study of the inverse loading of a three-dimensional helical spring. Furthermore, we develop a theory-assisted optimization strategy for cases in which the constrains of the undeformed configurations cannot be directly formulated as BCs. Using this strategy, we achieve rational inverse design of complex spatial curves and curve-discretized surfaces with varying Gaussian curvatures. Our theoretical predictions are validated through both discrete elastic rod simulations and experiments.

==> preamble.tex <==
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{physics}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage[left=23mm,right=13mm,top=35mm,columnsep=15pt]{geometry} 
\usepackage{adjustbox}
\usepackage{placeins}
\usepackage[T1]{fontenc}
\usepackage{lipsum}
\usepackage{csquotes}
